An artificial neural network approach to bifurcating phenomena in computational fluid dynamics

This work deals with the investigation of bifurcating fluid phenomena using a reduced order modelling setting aided by artificial neural networks. We discuss the POD-NN approach dealing with non-smooth solutions set of nonlinear parametrized PDEs. Thus, we study the Navier-Stokes equations describing: (i) the Coanda effect in a channel, and (ii) the lid driven triangular cavity flow, in a physical/geometrical multi-parametrized setting, considering the effects of the domain's configuration on the position of the bifurcation points. Finally, we propose a reduced manifold-based bifurcation diagram for a non-intrusive recovery of the critical points evolution. Exploiting such detection tool, we are able to efficiently obtain information about the pattern flow behaviour, from symmetry breaking profiles to attaching/spreading vortices, even at high Reynolds numbers.

==> nb_reg.tex <==

\subsubsection{The non-bifurcation regime}
Let us first consider the Navier-Stokes equations in the non bifurcating regime where the solution to the parametrized PDE exists and is unique. 

For this test case we have a one dimensional parameter space for the viscosity, namely $\mu \in \Pa = [2, 30]$ corresponding to $P = 1$ and we chose a maximum number of basis functions for both fields $u$ and $p$ corresponding to $N_u  = N_p = 10$. We remark that actually the dimension of the reduced basis space for the velocity is increased by one, due to the lifting coming from the inhomogeneous Dirichlet BC.
 
As concerns the  learning procedure through epochs, we started from $\eta_0 = 0.3$ for both networks and we updated it by means of the hyperbolic decay weighted by the square root in \eqref{learning_decay}, considering $N^{ep}_{it} = 5 \cdot 10^2$ and $N^{ep}_{\max} = 10^4$.

Once again, the offline phase is initialized with $N_{train} = n_b^2$ (and corresponding size $n_b$ for the mini-batches, where $n_b =6(i+1)$ with $i=1,2,3$) equispaced points in the parameter set $\Pa$, using the same ratio as before to split the dataset in train, test and validation sets.

%Given the lower dimension of the parameter space, the network is constructed only by means of $H_K = 15$ hidden neurons per layer.

%We present the decay of the velocity loss function for training and validating sets in Figure \ref{fig:loss_ns}.  In this case, the nonlinearity clearly complicates the setting, with an initial high value for both the loss functions. Despite this, we can see that already after the first 50 epochs the network learned the map from parameter to reduced coefficients and it is able to generalize for different values of the input.
%
%\begin{figure}
%\centering   
%\includegraphics[width=6.5cm]{Loss_epoch_ns.eps}   
%\caption{Training and validation loss function for the velocity field with respect to each epoch.}  
%\label{fig:loss_ns}   
%\end{figure} 

We tested the network accuracy properties on $\Xi_{te}$ with respect to the dimension of the dataset, while increasing the number of hidden layers $L_K$ and of hidden neurons $H_K$.
Thus, in Figure \ref{fig:err_NS} we show a comparison of the mean NN errors $\overline{\epsilon}_{NN}$ for the velocity and pressure fields with respect to the number $H_K$ of neurons for different numbers of hidden layer employed.

\begin{figure}
\begin{minipage}{0.45\textwidth}
\centering   
\includegraphics[width=6cm]{error_velocity.pdf}   
\label{fig:err_NS_v}   
\end{minipage}
\begin{minipage}{0.45\textwidth}
\centering   
\includegraphics[width=6cm]{error_pressure.pdf}   
\label{fig:err_NS_p}   
\end{minipage}
\caption{Mean NN errors $\overline{\epsilon}_{NN}$ for velocity and pressure fields, left and right respectively.}
\label{fig:err_NS}
\end{figure}


In Figures \ref{fig:err_nn_ns_new}, \ref{fig:err_nn_ns_p_new} we show the error $\epsilon_{NN}(\boldsymbol{\mu})$ computed for the parameters $\boldsymbol{\mu}$ belonging to $\Xi_{te}$ for the velocity and the pressure. 
Also for this nonlinear problem, in the best case scenario, we were able to gain good approximation properties. In fact, we obtained for the velocity field $\epsilon^{\max}_{NN} = 0.000369$ as the maximum error (near the left extrema of the parameter set $\Pa$, where we approach to the bifurcation point), and $\overline{\epsilon}_{NN} = 0.00012$ as the mean error over the testing dataset. Similar considerations hold for the pressure field, where again an increased error is observed mostly while approaching to lower values of the viscosity. We remark that such region is characterized by flow with increasing flux and of course it has to be properly represented inside the training set $\Xi_{tr}$ after the splitting.

\begin{figure}
\centering  
\begin{minipage}{0.45\textwidth}
\centering   
\includegraphics[width=6cm]{ANN_error_ns.pdf}   
\caption{Error $\epsilon_{NN}(\mu)$ for the velocity field $u$ computed on $\Xi_{te}$.}
\label{fig:err_nn_ns_new}
\end{minipage}\qquad
\begin{minipage}{0.45\textwidth}
\centering   
\includegraphics[width=6cm]{ANN_pressure_error.pdf}   
\caption{Error $\epsilon_{NN}(\mu)$ for the pressure field $p$ computed on $\Xi_{te}$.}  
\label{fig:err_nn_ns_p_new}  
\end{minipage} 
\end{figure} 

We show in Figures \ref{fig:NS_sol_hf}, \ref{fig:NS_sol_rb} and \ref{fig:NS_sol_nn} a representative solution obtained with the FE method, RB method and POD-NN technique. 
Moreover, we show the corresponding errors with respect to the FE solution in Figures \ref{fig:err_NS_sol_v} and \ref{fig:err_NS_sol_p}, respectively for velocity and pressure fields, using both the RB and the POD-NN strategies.
 
\begin{figure}
\centering   
\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=10cm]{NS_sol_hf}   
\caption{High fidelity}  
\label{fig:NS_sol_hf}   
\end{subfigure} 
\begin{subfigure}[b]{\textwidth}
\centering   
\includegraphics[width=10cm]{NS_sol_rb}   
\caption{Reduced basis}  
\label{fig:NS_sol_rb}   
\end{subfigure} 
\begin{subfigure}[b]{\textwidth}
\centering   
\includegraphics[width=10cm]{NS_sol_nn}   
\caption{POD-NN} 
\end{subfigure} 
\caption{Comparison between velocity field for the Navier-Stokes system with $\mu = 2.66$}
\label{fig:NS_sol_nn}   
\end{figure} 

 
\begin{figure}
\centering   
\includegraphics[width=10cm]{err_NS_sol_rb_v}
\includegraphics[width=10cm]{err_NS_sol_nn_v}
\caption{Relative errors HF-RB (top) and HF-NN (bottom) on the velocity field for the Navier-Stokes problem with $\mu = 4.09$.}
\label{fig:err_NS_sol_v}
\end{figure}

\begin{figure}
\centering   
\includegraphics[width=10cm]{err_NS_sol_rb_p}
\includegraphics[width=10cm]{err_NS_sol_nn_p}
\caption{Relative errors HF-RB (top) and HF-NN (bottom) on the pressure field for the Navier-Stokes problem with $\mu = 4.09$.}
\label{fig:err_NS_sol_p}
\end{figure}



%In Figures \ref{fig:err_rb_ns}, \ref{fig:err_nn_ns} we show the error $\epsilon_{RB}(\boldsymbol{\mu})$ and $\epsilon_{NN}(\boldsymbol{\mu})$ computed for the parameters $\boldsymbol{\mu}$ belonging to $\Xi_{te}$. The low dimensionality of the parameter space allows us to have better results in terms of error analysis, in fact we obtain $\epsilon_{max} = 0.01121$ as the maximum error (near the left extrema of the parameter set, where we approach to the bifurcation point), and $\overline{\epsilon}_{NN} = 0.00301$ as the mean error over the testing dataset.
%\begin{figure}
%\begin{minipage}{0.45\textwidth}
%\centering   
%\includegraphics[width=6cm]{RB_error_ns.eps}   
%\caption{Error $\epsilon_{RB}(\boldsymbol{\mu})$ computed on $\Xi_{te}$.}  
%\label{fig:err_rb_ns}   
%\end{minipage}\hfill
%\begin{minipage}{0.48\textwidth}
%\centering   
%\includegraphics[width=6cm]{ANN_error_nns.eps}   
%\caption{Error $\epsilon_{NN}(\boldsymbol{\mu})$ computed on $\Xi_{te}$ .}  
%\label{fig:err_nn_ns}  
%\end{minipage} 
%\end{figure} 
 
Finally, the speed-up for the evaluation of the network on $\Xi_{te}$, with respect to the FE method is almost $1.2\cdot 10^6$, while the RB one is equal to $1.25$. This is consistent with the results obtained in the previous section, but we notice also that the gap between the two speed-ups increased. Indeed, the nonlinearity of the problem together with the lack of an efficient hyper-reduction/tensor assembly for the weak form, causes the standard RB approach to be characterized by a $\N$-dependent online phase.
In particular, the (actually unfair) comparison between intrusive and non-intrusive strategy, shows a difference of five orders of magnitude. 

